Uncertainty-guided Model Generalization to Unseen Domains

We study a worst-case scenario in generalization: Out-of-domain generalization from a single source. The goal is to learn a robust model from a single source and expect it to generalize over many unknown distributions. This challenging problem has been seldom investigated while existing solutions suffer from various limitations. In this paper, we propose a new solution. The key idea is to augment the source capacity in both input and label spaces, while the augmentation is guided by uncertainty assessment. To the best of our knowledge, this is the first work to (1) access the generalization uncertainty from a single source and (2) leverage it to guide both input and label augmentation for robust generalization. The model training and deployment are effectively organized in a Bayesian meta-learning framework. We conduct extensive comparisons and ablation study to validate our approach. The results prove our superior performance in a wide scope of tasks including image classification, semantic segmentation, text classification, and speech recognition.

==> tex_abstract.tex <==
\begin{abstract}

We study a worst-case scenario in generalization: Out-of-domain generalization from a single source. The goal is to learn a robust model from a single source and expect it to generalize over many unknown distributions. This challenging problem has been seldom investigated while existing solutions suffer from various limitations. In this paper, we propose a new solution. The key idea is to augment the source capacity in both input and label spaces, while the augmentation is guided by uncertainty assessment. To the best of our knowledge, this is the first work to (1) access the generalization uncertainty from a single source and (2) leverage it to guide both input and label augmentation for robust generalization.
The model training and deployment are effectively organized in a Bayesian meta-learning framework. 
We conduct extensive comparisons and ablation study to validate our approach. The results prove our superior performance in a wide scope of tasks including image classification, semantic segmentation, text classification, and speech recognition.\footnote{We provide source codes and pre-trained models in supplementary to reproduce the reported results.}

% We study a new problem called uncertain Out-of-domain generalization.
% domain generalization, uncertainty assessment, data augmentation, Bayesian meta-learning

%We aim at learning a robust model from a single domain and expect it to generalize over a \textit{unknown} domain distribution. We propose a new method named uncertainty-guided out-of-domain inference to solve this problem. The key idea is to increase the domain capacity in both input and label space. We propose uncertainty-guided feature perturbations to yield domain-knowledge-free augmentation. The uncertainty encoded in domain augmentation can further provide guidance to learnable mixup for label space augmentation, and enable fast uncertainty estimation. Finally, we propose a novel Bayesian meta-learning framework to maximize the posterior distribution of domain augmentation, such that the learned model can generalize well on unseen domains. We show that our method achieves superior performance on a wide scope of tasks, including \textit{image classification}, \textit{text classification}, and \textit{speech recognition}. We show that our method achieves superior performance on a wide scope of tasks, including \textit{image classification}, \textit{text classification}, and \textit{speech recognition}.\footnote{We provide source codes and pre-trained models in supplementary to reproduce the reported results.}

\end{abstract}
